Incomplete Contracting and AI Alignment

We suggest that the analysis of incomplete contracting developed by law and economics researchers can provide a useful framework for understanding the AI alignment problem and help to generate a systematic approach to finding solutions. We first provide an overview of the incomplete contracting literature and explore parallels between this work and the problem of AI alignment. As we emphasize, misalignment between principal and agent is a core focus of economic analysis. We highlight some technical results from the economics literature on incomplete contracts that may provide insights for AI alignment researchers. Our core contribution, however, is to bring to bear an insight that economists have been urged to absorb from legal scholars and other behavioral scientists: the fact that human contracting is supported by substantial amounts of external structure, such as generally available institutions (culture, law) that can supply implied terms to fill the gaps in incomplete contracts. We propose a research agenda for AI alignment work that focuses on the problem of how to build AI that can replicate the human cognitive processes that connect individual incomplete contracts with this supporting external structure.

==> Incomplete Contracts/Old/pieces.tex <==
But this is complicated.  One problem is to determine which human(s) to include in the welfare function.  The owner of a self-driving car, for example, should obviously be included. But so too should passengers, pedestrians and bicyclists, the drivers and passengers in other vehicles, the owners of property potentially damaged by a car crash, and so on.  Human behavior is subject by a multitude of norms and laws precisely in order to ensure that humans are aligned with the well-being of other humans. So AI alignment requires that AIs built using reinforcement learning or neural nets that are subject to at least some behavioral rules specified \textit{a priori}.


\begin{itemize}
    \item the \textit{ex ante} specification versus \textit{ex post} negotiation tradeoff: \textit{ex post} adjustment can require paying off the agent, it may not be possible to commit not to renegotiate and this can influence strategic behavior of agent
    \item paying off an artificial agent may require designing rewards that incorporate payoff to change utility function, adopt action that is not optimal according to original utility function (human agents always have utility functions that value monetary payoff and this is routinely the solution for adjustment or contract design), this will face strategic risk that robot takes actions to secure buyout/payoff 
    \item rewards may need to be designed to elicit private information; robots may have incentives to lie/hide information just like human agents--see the design of revelation mechanisms, screening and signaling models--these models design menus of options that impose a cost on announcing a particular type (information set) and can get separation because cost is higher for some types than other--so an agent with low type, for example, finds it more costly than agent with high type to take costly action to announce 'I'm a high type' who gets higher reward
    \item multitasking and measurement problems--if you want A and B but can  measure/reward A better than B, you don't want to design the reward for A as if this were the only goal; this will distort behavior away from the harder to reward B.
    \item task allocation between human and robot should not necessarily just follow relative competence, task allocation creates incentives for learning/investment in information--literature shows that the allocation to actor with higher marginal impact on outcome is optimal
    \item the potential for human override can distort robot incentives to learn, take actions--this is analogous to the problem of real and formal authority in incomplete contracting (aghion tirole 1997)
    \item there may be value to recourse to third-party adjudicators to resolve gaps and ambiguities in rewards and resolve conflicts/disputes between human and robot--between \textit{ex ante} and \textit{ex post} utility functions--that is, for the robot's reward to actually be based on third-party variables (decisions, inputs).  In fact third-party adjudicators may be essential to reconcile the incomplete specification of constraints that arise from norms and laws and conflicts between endowed utility functions designed by particular humans and the interests of other humans
\end{itemize}


property rights (control over value rights--ability to take unilateral action to achieve value) and decision rights



\cite{Hadfield-Menell:2017}. As a result, they argue, developers may need to endow robots with reward functions that incentivize them to value human oversight.  They show that a robot that is, for example, uncertain about its reward function may determine that the action that optimizes expected reward is to seek further information from a human before acting.  Here we argue more generally that humans may need to design reward functions that incentivize robots to ensure that their current estimate of the human's utility function is equal to true utility. We may need to design rewards specifically with attention to the risk that the robot will, like OpenAI's boat-racing system, discover loopholes to exploit. \


==> Incomplete Contracts/author.tex <==
\author{
  Gillian K. Hadfield
  \thanks{Faculty Affiliate, Center for Human-Compatible Artificial Intelligence} \\
  Law School and Department of Economics\\
  University of Southern California\\
  Los Angeles, CA 90089 \\
  \texttt{ghadfield@law.usc.edu} 
  \And Dylan Hadfield-Menell \hspace{1cm} 
   \thanks{OpenAI} \\
   Department of Electrical Engineering and Computer Science\\
   Center for Human-Compatible Artificial Intelligence\\
   University of California\\
   Berkeley, CA 94720\\
   \texttt{dhm@eecs.berkeley.edu}
   \And Daniel Filan\\
    Department of Electrical Engineering and Computer Science\\
    Center for Human-Compatible Artificial Intelligence\\
   University of California\\
   Berkeley, CA 94720\\
   \texttt{daniel\_filan@berkeley.edu} \\
   \AND Stuart J. Russell\\
   Department of Electrical Engineering and Computer Science\\
   Center for Human-Compatible Artificial Intelligence\\
   University of California\\
   Berkeley, CA 94720\\
   \texttt{russell@cs.berkeley.edu} \\
   }

==> Old/pieces.tex <==
But this is complicated.  One problem is to determine which human(s) to include in the welfare function.  The owner of a self-driving car, for example, should obviously be included. But so too should passengers, pedestrians and bicyclists, the drivers and passengers in other vehicles, the owners of property potentially damaged by a car crash, and so on.  Human behavior is subject by a multitude of norms and laws precisely in order to ensure that humans are aligned with the well-being of other humans. So AI alignment requires that AIs built using reinforcement learning or neural nets that are subject to at least some behavioral rules specified \textit{a priori}.


\begin{itemize}
    \item the \textit{ex ante} specification versus \textit{ex post} negotiation tradeoff: \textit{ex post} adjustment can require paying off the agent, it may not be possible to commit not to renegotiate and this can influence strategic behavior of agent
    \item paying off an artificial agent may require designing rewards that incorporate payoff to change utility function, adopt action that is not optimal according to original utility function (human agents always have utility functions that value monetary payoff and this is routinely the solution for adjustment or contract design), this will face strategic risk that robot takes actions to secure buyout/payoff 
    \item rewards may need to be designed to elicit private information; robots may have incentives to lie/hide information just like human agents--see the design of revelation mechanisms, screening and signaling models--these models design menus of options that impose a cost on announcing a particular type (information set) and can get separation because cost is higher for some types than other--so an agent with low type, for example, finds it more costly than agent with high type to take costly action to announce 'I'm a high type' who gets higher reward
    \item multitasking and measurement problems--if you want A and B but can  measure/reward A better than B, you don't want to design the reward for A as if this were the only goal; this will distort behavior away from the harder to reward B.
    \item task allocation between human and robot should not necessarily just follow relative competence, task allocation creates incentives for learning/investment in information--literature shows that the allocation to actor with higher marginal impact on outcome is optimal
    \item the potential for human override can distort robot incentives to learn, take actions--this is analogous to the problem of real and formal authority in incomplete contracting (aghion tirole 1997)
    \item there may be value to recourse to third-party adjudicators to resolve gaps and ambiguities in rewards and resolve conflicts/disputes between human and robot--between \textit{ex ante} and \textit{ex post} utility functions--that is, for the robot's reward to actually be based on third-party variables (decisions, inputs).  In fact third-party adjudicators may be essential to reconcile the incomplete specification of constraints that arise from norms and laws and conflicts between endowed utility functions designed by particular humans and the interests of other humans
\end{itemize}


property rights (control over value rights--ability to take unilateral action to achieve value) and decision rights



\cite{Hadfield-Menell:2017}. As a result, they argue, developers may need to endow robots with reward functions that incentivize them to value human oversight.  They show that a robot that is, for example, uncertain about its reward function may determine that the action that optimizes expected reward is to seek further information from a human before acting.  Here we argue more generally that humans may need to design reward functions that incentivize robots to ensure that their current estimate of the human's utility function is equal to true utility. We may need to design rewards specifically with attention to the risk that the robot will, like OpenAI's boat-racing system, discover loopholes to exploit. \


==> author.tex <==
\author{
  Gillian K. Hadfield
  \thanks{Faculty Affiliate, Center for Human-Compatible Artificial Intelligence} \\
  Law School and Department of Economics\\
  University of Southern California\\
  Los Angeles, CA 90089 \\
  \texttt{ghadfield@law.usc.edu} 
  \And Dylan Hadfield-Menell \hspace{1cm} 
   \thanks{OpenAI} \\
   Department of Electrical Engineering and Computer Science\\
   Center for Human-Compatible Artificial Intelligence\\
   University of California\\
   Berkeley, CA 94720\\
   \texttt{dhm@eecs.berkeley.edu}
   \And Daniel Filan\\
    Department of Electrical Engineering and Computer Science\\
    Center for Human-Compatible Artificial Intelligence\\
   University of California\\
   Berkeley, CA 94720\\
   \texttt{daniel\_filan@berkeley.edu} \\
   \AND Stuart J. Russell\\
   Department of Electrical Engineering and Computer Science\\
   Center for Human-Compatible Artificial Intelligence\\
   University of California\\
   Berkeley, CA 94720\\
   \texttt{russell@cs.berkeley.edu} \\
   }
